Training-Free Robust Multimodal Learning via Sample-Wise Jacobian Regularization

Multimodal fusion emerges as an appealing technique to improve model performances on many tasks. Nevertheless, the robustness of such fusion methods is rarely involved in the present literature. In this paper, we propose a training-free robust late-fusion method by exploiting conditional independence assumption and Jacobian regularization. Our key is to minimize the Frobenius norm of a Jacobian matrix, where the resulting optimization problem is relaxed to a tractable Sylvester equation. Furthermore, we provide a theoretical error bound of our method and some insights about the function of the extra modality. Several numerical experiments on AV-MNIST, RAVDESS, and VGGsound demonstrate the efficacy of our method under both adversarial attacks and random corruptions.

==> Multimodal-Jacob-ECCV2022-for-arxiv (1)/background.tex <==
\section{Preliminary}\label{sec:background}

\textbf{Network Robustness}\quad To verify network robustness, two major kinds of perturbations are used, which in our paper we referred to as (i) adversarial attacks such as FGSM, PGD, or CW attack \cite{goodfellow2014fsgm,madry2017towards_resist_attack,carlini2017cw} and (ii) random corruptions such as Gaussian noise, missing entries or illumination change \cite{stab_train,kim2019single}. Correspondingly, many methods have been proposed to offset the negative effects of such perturbations. Adversarial training based on projected gradient descent \cite{madry2017towards_resist_attack} is one strong mechanism to defend against adversarial attacks, and the recent Free-m method \cite{shafahi2019freem} is proposed as its fast variant. Besides adversarial training, several regularization techniques are also proven to have such capability, such as Mixup \cite{zhang2020mixup1}, Jacobian regularization \cite{jacobian2}. Alternatively, with regard to random corruptions, Mixup and Jacobian regularization are also effective in this case \cite{zhang2017mixup2,jacobian3}. Another powerful approach is stability training \cite{stab_train}, where it introduces an additional KL divergence term into the conventional classification loss so that the trained DNNs are stabilized.

\vspace{6pt}

\noindent\textbf{Multimodal Learning}\quad DNNs trained by fusing data from different modalities have outperformed their unimodal counterparts in various applications, such as object detection \cite{stat_fusion2,kim2019single}, semantic segmentation \cite{chen2020bi_semantic_seg2,feng2020deep_sementic_seg1}, audio recognition \cite{gemmeke2017audio1,chen2020vggsound}. Based on where the information is exchanged between different modalities, multimodal fusion methods could be classified into three kinds: (i) early-fusion \cite{wagner2016multispectral,stat_fusion2}, (ii) middle-fusion \cite{kim2019single,deep_mm_channel_exchange}, and (iii) late-fusion \cite{stat_fusion2,liu2021one}. For instance, if the information is fused at the end of DNNs (e.g., Figure \ref{fig:illsutration_of_method}), such a method belongs to the late-fusion category.

Although vast efforts have been put into exploiting multimodal fusion methods to improve DNNs' accuracy on specific learning tasks, few works have explored network robustness in the multimodal context. Specifically, \cite{mees2016adaptive1}, \cite{valada2017adaptive2}, and \cite{kim2018robust} exploited gating networks to deal with random corruptions, adverse or changing environments. Afterwards, \cite{kim2019single} proposed a surrogate minimization scheme and a latent ensemble layer to handle single-source corruptions. However, all the aforementioned methods belong to middle-fusion and only random corruptions are considered. On the other hand, we focus on another important scenario: late-fusion, and besides corruptions, we further take adversarial attacks into account. To the best of our knowledge, robust late-fusion is un-explored in the previous literature.

==> Multimodal-Jacob-ECCV2022-for-arxiv (1)/conclusion.tex <==
\section{Discussion and Future Work}\label{sec:conclusion}
In this paper, we propose a training-free robust late-fusion method. Intuitively, our method designs a filter for each sample during inference (i.e., test time). Such a filter is implemented by Jacobian regularization, and after a sample goes through it, the change of final multimodal prediction is limited to some amount under an input perturbation. The error bound analysis and series of experiments justify the efficacy of our method both theoretically and numerically. The Twomoon example explains the biasing effect of the extra modality, rooted for the difference between unimodal and multimodal. 

Our method opens up other directions for further exploration. In the unimodal context, we understand that directly applying our method usually doesn't change the prediction. Thus, would it be capable to adjust the confidence of a DNN? Another possibility is that besides $\mathbf{W}_x$, we deliberately add another bias term $\mathbf{b}_x$ and optimize both for unimodal robustness. Alternatively, in the multimodal context, we might consider minimizing the derivative of the final prediction directly to the input feature. Moreover, it is educational to compare it with consistency regularization. Last but not least, statistical fusion implicitly uses the assumption that train and test data come from the same distribution, so that we could calculate $\mathbf{freq}$ based on the train dataset and reuse it in inference time. When domain shift presents, this doesn't work and a straightforward remedy might be to make $\mathbf{freq}$ a learnable parameter.

==> Multimodal-Jacob-ECCV2022-for-arxiv (1)/intro.tex <==
\section{Introduction}

Deep fusion models have recently drawn great attention of researchers in the context of multimodal learning \cite{vielzeuf2018centralnet,mm_survey,perez2019mfas,deep_mm_channel_exchange,xue2021multimodal} as it provides an easy way to boost model accuracy and robustness. For instance, RGB cameras and LiDARs are usually deployed simultaneously on an autonomous vehicle, and the resulting RGB images and point clouds are referred to as two modalities, respectively. When RGB images are blurry at night, point clouds could provide complementary information and help to make decisions in vision tasks \cite{kim2019single}. Over the past few years, numerous multimodal fusion methods have been proposed at different levels: early-, middle-, and late-fusion \cite{stat_fusion2}. In early-fusion, input feature vectors from different modalities are concatenated and fed into one single deep neural network (DNN), while in middle-fusion, they go into DNNs independently and exchange information in feature space. Unlike the previous two cases, late-fusion is realized by merging distinct DNNs at their output layers via concatenation, element-wise summation, etc. 

These three levels of fusion possess different pros and cons. For instance, late-fusion, the primary concern of our paper, is (i) privacy-friendly and (ii) convenient to deploy. Specifically, assume that a hospital wants to have an AI agent to judge whether a patient has a certain disease or not \cite{sun2020tcgm}. It has to divide the complete training feature (e.g., medical records, X-ray images) of every patient and deliver them to different AI companies, otherwise, the patients' identities will be exposed and their privacy are unprotected. This, in turn, directly rules out the possibility of applying early- or middle-fusion methods. On the other hand,  the hospital could still exploit late-fusion technique to generate the ultimate AI agent after several unimodal DNNs are trained by AI companies. Moreover, unlike early- or middle-fusion, many late-fusion methods could tolerate missing modality information (i.e., no need for paired training data) and thus are convenient to deploy.

Although late-fusion is a mature topic in the literature, its performance under adversarial attacks \cite{madry2017towards_resist_attack,robust_at_odds} and random corruptions \cite{stab_train,kim2019single} is rather under-explored. In this paper, we address the problem of robust late-fusion by utilizing Jacobian regularization \cite{jacobian4,jacobian2,jacobian3,jacobian1} and conditional independence assumption \cite{sun2020tcgm}. The key is to minimize the Frobenius norm of a Jacobian matrix so that the multimodal prediction is stabilized (see Figure \ref{fig:illsutration_of_method}). Our main contributions are as follows:
\begin{itemize}
    \item To the best of our knowledge, we are the first to propose a training-free robust late-fusion method. The involving optimization problem is relaxed to a Sylvester equation \cite{solve_sylvester1}, and the solution is obtained with only a little computational overhead.
    \item We provide a theoretical error bound of our proposed robust late-fusion method and an illustrative explanation about the function of the extra modality via the TwoMoon example.
    \item Thorough numerical experiments demonstrate that our method outperforms other late-fusion methods and is capable to handle both adversarial attacks and random corruptions.
\end{itemize}

% We briefly review the background of adversarial training and multimodal learning in Section \ref{sec:background}. Next, we describe the proposed method in Section \ref{sec:method1} and explain the function of the extra modality in Section \ref{sec:method2}. Several numerical experiments are presented to verify the efficacy of our method in Section \ref{sec:experiment}, and finally we conclude in Section \ref{sec:conclusion}.

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/Picture1.pdf}
    \caption{Illustration of the proposed robust late-fusion method. Before unimodal raw logit $\mathbf{z}_A$ and $\mathbf{z}_B$ are fused, the Jacobian regularization technique is applied. Roughly speaking, it will enforce the derivative of $\mathbf{p}$ with respect to $\mathbf{z}_A$ becomes smaller. Thus, when $\mathbf{z}_A$ is perturbed to $\mathbf{z}_A^{\prime}$ (due to random corruption or adversarial attack), the change of multimodal prediction $||\mathbf{p}^\prime-\mathbf{p}||$ will be limited to some extent. For illustration purpose, all variables here (e.g., $\mathbf{p},\mathbf{z}_A$) are drawn in one-dimensional space.}
    \label{fig:illsutration_of_method}
\end{figure}

==> Multimodal-Jacob-ECCV2022-for-arxiv (1)/method.tex <==
\section{Sample-Wise Jacobian Regularization}\label{sec:method1}
Consider a supervised $K$-class classification problem in the multimodal context. Suppose that features from two distinct modalities $A$ (e.g., audio) and $B$ (e.g., video) are provided in the form of $\mathcal{D}_A=\{(\mathbf{x}^i_A,{y}^{i})\}_{i=1}^N$ and $\mathcal{D}_B=\{(\mathbf{x}^i_B,{y}^{i})\}_{i=1}^N$, where $\{\mathbf{x}_A,\mathbf{x}_B\}$ represents input features and ${y}\in\{0,1,\cdots,K-1\}$ represents the true label. We train two unimodal networks separately, each corresponding to one modality. Given a specific input feature $\mathbf{x}_A$, the first unimodal network calculates the class prediction $\mathbf{p}_A\in\mathbb{R}^K$ by:
\begin{equation}\label{eq:expression_final_layer}
    \mathbf{p}_A=\bm\sigma_1(\mathbf{z}_A)=\bm\sigma_1(\mathbf{W}_A\mathbf{h}_A+\mathbf{b}_A)=\bm\sigma_1(\mathbf{W}_A\mathbf{f}_A(\mathbf{x}_A)+\mathbf{b}_A)
\end{equation}
where $\bm\sigma_1(\cdot)$ represents the Softmax function, $\mathbf{z}_A\in\mathbb{R}^K$ represents the raw logit, and $\mathbf{h}_A=\mathbf{f}_A(\mathbf{x}_A)\in\mathbb{R}^{H}$ represents the feature being fed into the last layer \footnote{(\ref{eq:expression_final_layer}) holds because the last layer is usually implemented as a fully connected (FC) layer with Softmax activation in classification tasks.}. Here $\mathbf{W}_A\in\mathbb{R}^{K\times H}$ and $\mathbf{b}_A\in\mathbb{R}^K$ are the learnable weight and bias of the last linear layer, respectively. Similarly, the second unimodal network provides the class prediction $\mathbf{p}_B=\bm\sigma_1(\mathbf{z}_B)=\bm\sigma_1(\mathbf{W}_B\mathbf{h}_B+\mathbf{b}_B)=\bm\sigma_1(\mathbf{W}_B\mathbf{f}_B(\mathbf{x}_B)+\mathbf{b}_B)$.

Based on the conditional independence assumption \cite{stat_fusion1}, the basic statistical late-fusion method generates the final class prediction as \cite{stat_fusion2}:
\begin{equation}\label{eq:expression_stat_fusion}
    \mathbf{p}=\bm\sigma_2(\frac{\mathbf{p}_A\odot\mathbf{p}_B}{\mathbf{freq}})=\bm\sigma_2(\frac{\bm\sigma_1(\mathbf{z}_A)\odot\bm\sigma_1(\mathbf{z}_B)}{\mathbf{freq}})
\end{equation}
where the division is performed in an element-wise manner,  $\odot$ represents the element-wise product, and $\bm\sigma_2(\cdot)$ represents a linear normalization enforcing the summation of elements equal to one. Here $\mathbf{freq}\in\mathbb{R}^K$ contains the occurring frequencies of each class, calculated from the training dataset.

Our proposed approach builds upon (\ref{eq:expression_stat_fusion}). Specifically, we consider adding two $K\times K$ weight matrices $\{\mathbf{W}_a,\,\mathbf{W}_b\}$ ahead of $\{\mathbf{z}_A,\,\mathbf{z}_B\}$, respectively, right before they get activated. Consequently, the final multimodal prediction is re-calibrated as:
\begin{equation}\label{eq:expression_p_prime}
    \mathbf{p}^\prime=\bm\sigma_2(\frac{\bm\sigma_1(\mathbf{z}_A^\prime)\odot\bm\sigma_1(\mathbf{z}_B^\prime)}{\mathbf{freq}})=\bm\sigma_2(\frac{\bm\sigma_1(\mathbf{W}_a\mathbf{z}_A)\odot\bm\sigma_1(\mathbf{W}_b\mathbf{z}_B)}{\mathbf{freq}})
\end{equation}
Suppose that the data provided from modality $A$ are perturbed at the input or feature level, while the data from modality $B$ are clean. For matrix $\mathbf{W}_b$, we could simply set it to an identity matrix, implying that we didn't invoke the robust add-on for the second modality. To determine the value of $\mathbf{W}_a$, we first calculate the derivative of $\mathbf{p}^\prime$ with respect to $\mathbf{h}_A$ (See Supplementary):
\begin{equation}\label{eq:derivative}
    \frac{\partial \mathbf{p}^\prime}{\partial \mathbf{h}_A}= \mathbf{J}^\prime\mathbf{W}_a\mathbf{W}_A=[\mathbf{p}^\prime\mathbf{p}^{\prime,T}-\text{Diag}(\mathbf{p}^\prime)]\mathbf{W}_a\mathbf{W}_A
\end{equation}
Then we minimize the following regularized Jacobian loss with respect to $\mathbf{W}_a$:
\begin{equation}\label{eq:expression_loss}
     \min_{\mathbf{W}_a}\ L =\min_{\mathbf{W}_a}\ (1-\gamma) ||\mathbf{J}^\prime\mathbf{W}_a\mathbf{W}_A||^2_F + \gamma ||\mathbf{W}_a-\mathbf{I}||_F^2
\end{equation} 
where $0<\gamma<1$ is a tunable hyper-parameter. Minimizing the first term in the loss could make the change of $\mathbf{p}^\prime$ limited to some extent when $\mathbf{h}_A$ is perturbed, while the second term in the loss guarantees numerical stability and the prediction in the perturbed case won't get too far from that of the clean case. For a specific multimodal input $\{\mathbf{x}_A,\mathbf{x}_B\}$, once $\mathbf{W}_a$ is determined, so are $\mathbf{p}^\prime$ and $\mathbf{J}^\prime$ via (\ref{eq:expression_p_prime}) and (\ref{eq:derivative}), respectively. Thus, (\ref{eq:expression_loss}) is well-determined and non-linear with respect to $\mathbf{W}_a$. 

\begin{algorithm}
\caption{Iteratively solving regularized Jacobian loss}
\label{alg:solve_loss}
\begin{algorithmic}[1]
\STATE {Given one specific input $\{\mathbf{x}_A,\mathbf{x}_B\}$. Initialize iteration index $t=0$.}
\STATE {Perform one forward pass, yielding the initial class prediction $\mathbf{p}^{(0)}$.}
\WHILE{$t<t_{\text{max}}$} 
\STATE {Calculate $\mathbf{J}^{(t)}=\mathbf{p}^{(t)}\mathbf{p}^{(t),T}-\text{Diag}(\mathbf{p}^{(t)})$.}
\STATE {Minimize $L^{(t)} = (1-\gamma) ||\mathbf{J}^{(t)}\mathbf{W}_a\mathbf{W}_A||^2_F + \gamma ||\mathbf{W}_a-\mathbf{I}||_F^2$ with respect to $\mathbf{W}_a$.}
\STATE {Calculate $\mathbf{p}^{(t+1)}$ based on Eq (\ref{eq:expression_p_prime}) with the optimal $\mathbf{W}_a$.}
\STATE {Update $t=t+1$.}
\ENDWHILE 
\STATE {Return $\mathbf{p}^\prime=\mathbf{p}^{(t)}$.}
\end{algorithmic}
\end{algorithm}



We propose a heuristic iterative method making the above optimization problem tractable in Algorithm \ref{alg:solve_loss}. Our key is to decouple $\mathbf{J}^\prime$ from $\mathbf{W}_a$. Namely, in step 5 of Algorithm \ref{alg:solve_loss}, all terms are known except $\mathbf{W}_a$, and thus the relaxed loss is convex. After writing out all terms of $\partial L^{(t)}/\partial \mathbf{W}_a$, we observe that it is a Sylvester equation \cite{solve_sylvester1}. It has a unique solution and the run time is as large as inverting a $K\times K$ matrix and hence affordable. See Supplementary for details. 

\vspace{6pt}

\noindent\textbf{Remarks}\quad First, in our implementation we find that one iteration could already yield a sufficiently accurate result, thus all our numerical results are reported with $t_{\text{max}}=1$ (i.e., $\mathbf{p}^\prime=\mathbf{p}^{(1)}$). Second, if we know data from modality $B$ are also perturbed, we could solve $\mathbf{W}_b$ in a similar manner. Third, notice that our approach is invoked merely during inference (i.e., test time), but not the train time. Furthermore, we demonstrate our approach in the context of two modalities, while obviously, it could be equally applied to many modalities. Finally, with a moderate assumption, we can further prove that when the input is perturbed, the change of final prediction enhanced by our method is limited to a certain amount. This has been summarized in Theorem \ref{theorem:change_output} (see Supplementary for details). Some immediate corollary include: (i) when $\bm{\epsilon}\sim N(\mathbf{0},\mathbf{\Sigma})$, the bound is simplified to  ${E}[||\mathbf{p}^{\prime,noise}-\mathbf{p}^\prime||]\leq l\,({\frac{\gamma K}{2(1-\gamma)}})^{1/2}\,\text{Tr}[\mathbf{\Sigma}]$, (ii) when the $L_2$ norm of $\bm{\epsilon}$ is constrained smaller than $\delta$ (usually assumed in adversarial attacks), the bound is simplified to $||\mathbf{p}^{\prime,noise}-\mathbf{p}^\prime||\leq l\,\delta\,({\frac{\gamma K}{2(1-\gamma)}})^{1/2}$.

\begin{theorem}\label{theorem:change_output}
If $\mathbf{f}_A$ is $l$-Lipschitz continuous and $\mathbf{x}_A$ is perturbed by $\bm{\epsilon}$: $\mathbf{x}_A^{\text{noise}}=\mathbf{x}_A+\bm{\epsilon}$, then the Euclidean norm of our final prediction (i.e., $||\mathbf{p}^{\prime,noise}-\mathbf{p}^\prime||$) at most changes $l\sqrt{\frac{\gamma K}{2(1-\gamma)}}||\bm\epsilon||$.
\end{theorem}

\section{Necessity of the Extra Modality: Biasing Effect}\label{sec:method2}
In this sub-section, we explain the principles behind our approach. Let us move one step back and consider the unimodal case. In what follows, we will demonstrate that our approach might not work well in the unimodal context, which in turn justifies the necessity of the extra modality.

At first glance, our approach seems to be equally applicable in the unimodal context. Namely, suppose that only one unimodal network $\mathbf{p}=\bm\sigma_1(\mathbf{z})=\bm\sigma_1(\mathbf{W}\mathbf{h}+\mathbf{b})$ is available, in test time and for each specific input $\mathbf{x}$, we add a weight matrix $\mathbf{W}_x$ before the raw logit $\mathbf{z}$ being fed into the Softmax activation, re-calibrating the final unimodal prediction as: $\mathbf{p}^\prime=\bm\sigma_1(\mathbf{z^\prime})=\bm\sigma_1(\mathbf{W}_x\mathbf{z})$. Here $\mathbf{W}_x$ can be solved by analogy to (\ref{eq:expression_loss}). However, we observe that the introduction of $\mathbf{W}_x$ usually won't change the final prediction. For an intuitive understanding, we consider the TwoMoon example used by \cite{xue2021multimodal}. In this example, all data points are scattered in a 2D space. The data located at the upper and lower leaf have true labels $0$ and $1$, and are colored by red and blue, respectively.

\begin{figure}[!htp]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/twomoon_um_final_version.pdf}
    \vspace{-18pt}
    \caption{({Unimodal case}) The leftmost figure reveals the results of training and testing on clean data. The heatmap in the background represents the value of $||\mathbf{J}\mathbf{W}||_F$. The remaining right three figures show the results of testing on data with Gaussian noise, and similarly, the heatmap in the background represents the value of $||\mathbf{J}\mathbf{W}_x\mathbf{W}||_F$. For each figure, the test accuracy on clean and noisy data are reported at the left top and right bottom.}
    \label{fig:twoomoon_um}
\end{figure}
In the unimodal case, we take both horizontal and vertical coordinates as input and train a neural network with three FC layers. As shown in Figure \ref{fig:twoomoon_um} (a), the network perfectly fits to the clean data and achieves 97.75\% accuracy on the clean test data. In the remaining three figures, we evaluate the trained network on noisy test data. Specifically, we deliberately choose $\gamma=1.0$ in Figure \ref{fig:twoomoon_um} (b), so that our approach is actually not invoked (since the solved $\mathbf{W}_x$ equals $\mathbf{I}$). In this case, the accuracy drops to 97.00\% on noisy data, while the heatmap in the background doesn't change at all compared to Figure \ref{fig:twoomoon_um} (a). In Figure \ref{fig:twoomoon_um} (c) and (d), we choose $\gamma=0.5$ and $\gamma=0.1$, respectively. We observe that even though the color of the heatmap surely becomes lighter as expected, the test accuracies of both cases are still 97.00\%. More importantly, we find that this phenomenon is not coincident and that the prediction doesn't change for any input after adding $\mathbf{W}_x$ in unimodal binary classification. See Supplementary for rigorous mathematical proof. Moreover, in a $K$-class ($K>2$) classification problem, the final prediction might change if $\gamma$ is sufficiently small. For instance, given $\mathbf{z}=[1,0,2]^T$ and $\mathbf{W}=\mathbf{I}$, if we choose $\gamma=0.5$, then the final prediction will change from $\mathbf{p}=[0.245, 0.090, 0.665]^T$ to $\mathbf{p}^\prime=[0.270,0.096,0.635]^T$, where the last entry remains to be the largest. However, if we choose $\gamma=0.01$, then the final prediction will become $\mathbf{p}^\prime=[0.391, 0.219, 0.390]^T$, and now the first entry is the largest. See Supplementary for a theoretical bound of $\gamma$ in this high-dimensional case.

% \begin{theorem}\label{thm:unimodal_2d}
% When $K=2$, adding $\mathbf{W}_x$ won't change the index of the largest value in the class predictions, i.e., $\text{argmax }\mathbf{p}^\prime=\text{argmax }\mathbf{p}$.
% \end{theorem}
% \begin{theorem}\label{thm:unimodal_high_dimensional}
% Without loss of generality, we assume $\mathbf{B}=(\mathbf{W}\mathbf{W}^T)^{-1}=\mathbf{I}$. Only when
% \begin{equation}
%     0 < \gamma < (\frac{1}{(3-1/K)\epsilon}+1)^{-1}
% \end{equation}
% the final prediction will change (i.e., $\text{argmax }\mathbf{p}^\prime\neq \text{argmax }\mathbf{p}$).
% \end{theorem}

Now we turn to the multimodal case. We treat the horizontal coordinates as one modality, and the vertical coordinates as the second modality. Two neural networks are trained, each corresponding to one modality. Then we fuse them based on the aforementioned statistical fusion method. As shown in Figure \ref{fig:twoomoon_mm}, in the multimodal context, when our method is invoked ($\gamma=0.5$ or $0.1$), the color of the heatmap becomes lighter and the test accuracies on noisy data all increase compared to the trivial statistical fusion (i.e., when $\gamma=1.0$). On the other hand, the test accuracies on clean data almost remain still (or slightly increase alongside $\gamma\downarrow$).

\begin{figure}[!htp]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/twomoon_mm_final_version.pdf}
    \vspace{-18pt}
    \caption{({Multimodal case}) The leftmost column reveals the results of training and testing on clean data. For illustration purpose, we only perturb the Y-coordinates with Gaussian noise. The first and second row correspond to small and large noise, respectively. Heatmaps reveal the values of $||\mathbf{J}\mathbf{W}||_F$ in (a) and $||\mathbf{J}\mathbf{W}_A\mathbf{W}||_F$ in (b), (c), and (d). For each figure, the test accuracy on clean and noisy data are reported at the left top and right bottom.}
    \label{fig:twoomoon_mm}
\end{figure}

\begin{lemma}\label{lemma:equi_stat_conc}
Statistical fusion is equivalent to concatenating the raw logits:
\begin{equation*}
   \bm\sigma_2(\frac{\mathbf{p}_A\odot\mathbf{p}_B}{\mathbf{freq}})=\bm\sigma_1(\mathbf{z}_A+\mathbf{z}_B-\ln\mathbf{freq})=\bm\sigma_1(
\left[
\begin{array}{cc}
     \mathbf{I} & \mathbf{I}\\
\end{array}\right]
\left[
\begin{array}{c}
     \mathbf{z}_A\\
     \mathbf{z}_B
\end{array}\right]
-\ln\mathbf{freq}) 
\end{equation*}
\end{lemma}

\noindent\textbf{Biasing effect of the extra modality}\quad As we have seen in the TwoMoon example, our proposed method behaves differently in the unimodal and multimodal context. To get a better understanding of this subtle difference, we first summarize an equivalent form of statistical fusion in Lemma \ref{lemma:equi_stat_conc} (see Supplementary). Now assume that the sample-wise $\mathbf{W}_a$ is added, then the final multimodal prediction becomes $\bm\sigma_1(\mathbf{W}_a\mathbf{z}_A+\mathbf{z}_B-\ln\mathbf{freq})$. Alternatively, in the unimodal context, our method adds a sample-wise $\mathbf{W}_x$ and the final prediction becomes $\bm\sigma_1(\mathbf{W}_x\mathbf{z})$. Comparing these two expressions, we observe that the introduced $\mathbf{W}_a$ and $\mathbf{W}_x$ occur ahead of the perturbed modality. In the unimodal case, the Softmax function $\bm\sigma_1$ directly applies onto $\mathbf{W}_x\mathbf{z}$, while in the multimodal case, the extra modality information $\mathbf{z}_B$ acts as a bias term inside the Softmax. Since entries of $\mathbf{z}_B$ have different values, it might impact the final prediction.

==> Multimodal-Jacob-ECCV2022-for-arxiv (1)/results.tex <==
\section{Experimental Results}\label{sec:experiment}
\subsection{AV-MNIST}

AV-MNIST \cite{perez2019mfas,vielzeuf2018centralnet} is a novel dataset created by pairing audio features to the original MNIST images. The first modality corresponds to MNIST images with size of $28\times 28$ and $75\%$ energy removed by principal component analysis \cite{perez2019mfas}. The second modality is made up of spectrograms with size of $112\times 112$. These spectrograms are extracted from audio samples obtain by merging pronounced digits and random natural noise. Following \cite{vielzeuf2018centralnet}, we use LeNet5 \cite{LeCun_handwritten} and a 6-layer CNN to process image and audio modalities, respectively. To thoroughly verify the efficiency of our method, we design various types of perturbations: (i) random corruptions including Gaussian noise ($\omega_0$), missing entries ($\omega_1$), and biased noise ($\omega_2,\omega_3$), and (ii) adversarial attacks including FGSM ($\omega_4$) and PGD attack ($\omega_5,\omega_6$). See Supplementary for detailed definitions.

\vspace{6pt}

\noindent\textbf{Baselines}\quad We limit our comparison to the range of late-fusion methods. To verify our method, we consider several methods which could improve network robustness, including (i) regular training, (ii) adversarial training (advT) by \cite{madry2017towards_resist_attack}, (iii) free-m training (freT) by \cite{shafahi2019freem}, (iv) stability training (stabT) by \cite{stab_train}, and (v) Mixup (mixT) by \cite{zhang2017mixup2}. To the best of our knowledge, no previous robust late-fusion methods exist. Thus for comparison purpose, we slightly modify the confidence-based weighted summation in \cite{xue_find_that_paper} and adapt it here, referred to as mean fusion with confidence-based weighted summation. Combinations of different fusion methods and robust add-ons provide us with a few baselines. We emphasize that in our experiments, the train data are always free of noise. Following \cite{kim2019single}, our experiments are mainly conducted on the case when one modality is perturbed. Results on various other settings are reported in Supplementary.

% \textbf{With trained unimodal networks}\quad We first consider the setting when unimodal networks are provided, and in test time, we attempt to directly fuse the predictions of both networks. This is preferred over training a multimodal network from scratch when time or data privacy is a major concern. 

% \begin{table}[!htbp]
%     \centering
%     \caption{Inference time of a StatFusNet is measured on a single GeForce RTX3090 with batch size $128$. The check mark $\checkmark$ represents which modality has been enhanced by our robust method.}
%     \label{table:run_time_of_solve_slv}
%     \begin{tabular}{cccc}
%     \toprule
%     \multirow{2}{*}{\quad}&
%     \multicolumn{2}{c}{Robust Add-on}&
%     \multirow{2}{*}{Inference Time (ms)} \\
%     \cline{2-3}
%       & Image & Audio & \\
%     \hline
%     StatFusNet1 &            &            & $5.87\,(1.0\times)$\\
%     StatFusNet2 & \checkmark &            & $14.16\,(2.4\times)$\\
%     StatFusNet3 &            & \checkmark & $12.99\,(2.2\times)$\\
%     StatFusNet4 & \checkmark & \checkmark & $22.04\,(3.8\times)$\\
%     \bottomrule
%     \end{tabular}
% \end{table}

% \begin{table}[!htbp]
% \small
% \centering
% \caption{Accuracies of different models (\%) are evaluated on AV-MNIST when audio features are perturbed. Mean accuracies are reported after repeatedly running 20 times. Each gray-shaded row in the statistical fusion subsection shares the same $\gamma$, and its value is selected from $\{0.1,0.5,0.9\}$. The green arrow \uu represents after applying our Jacobian regularization, the model accuracy increases compared to the corresponding counterpart without it, while the red arrow \dd represents decreasing.}
% \vspace{2pt}
% \begin{tabular}{cccccccccc}

% & (0,1)-w/o                                                              & $93.6$     & $80.4$          & $86.6$          & $89.9$          & $92.7$ \\
% \rowcolor{gray!20}\cellcolor{white} & (0,1)-w/{\color{gray!20}{o}}       & $94.7$ \uu & $84.5$ \uu      & $89.1$ \uu      & $92.2$ \uu      & $\bm{94.1}$ \uu \\
% & (0,2)-w/o                                                              & $91.7$     & $78.3$          & $83.5$          & $91.9$          & $92.4$ \\
% \rowcolor{gray!20}\cellcolor{white} & (0,2)-w/{\color{gray!20}{o}}       & $93.4$ \uu & $83.1$ \uu      & $86.4$ \uu      & $\bm{93.5}$ \uu & $93.7$ \uu \\
% Statistical & (0,3)-w/o                                                  & $93.0$     & $80.9$          & $87.7$          & $93.2$          & $93.2$ \\
% \rowcolor{gray!20}\cellcolor{white} Fusion & (0,3)-w/{\color{gray!20}{o}}& $93.0$ \uu & $82.3$ \uu      & $88.1$ \uu      & $92.7$ \dd      & $92.9$ \dd \\
% & (0,4)-w/o                                                              & $93.1$     & $83.7$          & $85.3$          & $83.4$          & $88.8$ \\
% \rowcolor{gray!20}\cellcolor{white}      & (0,4)-w/{\color{gray!20}{o}}  & $94.7$ \uu & $\bm{87.5}$ \uu & $87.8$ \uu      & $87.9$ \uu      & $91.9$ \uu \\
% & (0,5)-w/o                                                              & $95.1$     & $85.7$          & $\bm{90.1}$     & $91.1$          & $92.4$ \\
% \rowcolor{gray!20}\cellcolor{white} & (0,5)-w/{\color{gray!20}{o}}       & $95.0$ \dd & $86.1$ \uu      & $\bm{90.1}$ \dd & $91.0$ \dd      & $92.2$ \dd \\
% \midrule

% & (0,1)-w/o                                                              & $93.6$ & $80.3$ & $86.4$ & $89.8$ & $92.7$ \\
% \rowcolor{gray!20}\cellcolor{white} & (0,1)-w/{\color{gray!20}{o}}       & $90.5$ & $73.7$ & $83.6$ & $82.0$ & $88.2$ \\
% & (0,2)-w/o                                                              & $91.8$ & $78.3$ & $82.7$ & $91.9$ & $92.5$ \\
% \rowcolor{gray!20}\cellcolor{white} & (0,2)-w/{\color{gray!20}{o}}       & $86.0$ & $72.7$ & $77.5$ & $85.7$ & $86.9$ \\
% Mean & (0,3)-w/o                                                         & $93.0$ & $81.1$ & $87.7$ & $93.2$ & $93.2$ \\
% \rowcolor{gray!20}\cellcolor{white} Fusion & (0,3)-w/{\color{gray!20}{o}}& $82.4$ & $74.4$ & $78.6$ & $83.7$ & $83.5$ \\
% & (0,4)-w/o                                                              & $93.0$ & $83.8$ & $84.9$ & $83.5$ & $88.8$ \\
% \rowcolor{gray!20}\cellcolor{white} & (0,4)-w/{\color{gray!20}{o}}       & $90.9$ & $78.1$ & $81.8$ & $74.6$ & $81.3$ \\
% & (0,5)-w/o                                                              & $\bm{95.2}$ & $85.9$ & $89.7$ & $91.1$ & $92.5$ \\
% \rowcolor{gray!20}\cellcolor{white} & (0,5)-w/{\color{gray!20}{o}}       & $94.0$ & $82.1$ & $88.6$ & $87.1$ & $88.9$ \\
% \bottomrule

% \end{tabular}
% \label{table:exp_avmnist_gauss_moda1}
% \end{table}

\begin{table}[!ht]
\small
\centering
\caption{Accuracies of different models (\%) are evaluated on AV-MNIST when audio features are perturbed. Mean accuracies are reported after repeatedly running 20 times. The value of $\gamma$ is selected from $\{0.1,0.5,0.9\}$. The green \uu or red \dd arrow represents after applying our Jacobian regularization, the model accuracy increases or decreases compared to others with the same unimodal backbones. The best accuracy in one column is bolded. `UM' and `MM' represent `unimodal' and `multimodal', respectively. `MM($0,\,i$)' represents a multimodal network obtained by fusing the unimodal network indexed by `$0$' and `$i$'.}
\vspace{2pt}
\begin{tabular}{clcccccccc}
\toprule
UM / MM & ~~~~~Model &  Clean  & $\omega_0 = 1.0$ & $\omega_1 = 10$ &  $\omega_4 = 0.03$  &  $\omega_5 = 0.001$\\
\midrule
& 0: Img-regT       & $73.4$ & $73.4$ & $73.4$ & $73.4$ & $73.4$ \\
& 1: Aud-regT       & $83.9$ & $55.1$ & $73.3$ & $69.9$ & $77.8$ \\
UM   & 2: Aud-advT  & $84.4$ & $59.2$ & $72.0$ & $81.9$ & $83.3$ \\
Nets & 3: Aud-freT  & $82.1$ & $55.6$ & $71.9$ & $80.8$ & $81.6$ \\
& 4: Aud-staT       & $86.2$ & $67.6$ & $74.4$ & $66.5$ & $74.5$ \\
& 5: Aud-mixT       & $87.6$ & $61.3$ & $74.9$ & $74.9$ & $78.3$ \\
\midrule

&       Mean-w/o     & $93.6$     & $80.3$      & $86.4$      & $89.8$      & $92.7$ \\
MM &  Mean-w/        & $90.5$     & $73.7$      & $83.6$      & $82.0$      & $88.2$ \\
(0, 1) & Stat-w/o    & $93.6$     & $80.4$      & $86.6$      & $89.9$      & $92.7$ \\
&  Stat-w/ (ours)    & $94.7$ \uu & $84.5$ \uu  & $89.1$ \uu  & $92.2$ \uu  & $\bm{94.1}$ \uu \\

\hline
&       Mean-w/o     & $91.8$     & $78.3$      & $82.7$     & $91.9$          & $92.5$ \\
MM &  Mean-w/        & $86.0$     & $72.7$      & $77.5$     & $85.7$          & $86.9$ \\
(0, 2) & Stat-w/o    & $91.7$     & $78.3$      & $83.5$     & $91.9$          & $92.4$ \\
& Stat-w/ (ours)     & $93.4$ \uu & $83.1$ \uu  & $86.4$ \uu & $\bm{93.5}$ \uu & $93.7$ \uu \\

\hline
& Mean-w/o           & $93.0$     & $81.1$      & $87.7$     & $93.2$     & $93.2$ \\
MM & Mean-w/         & $82.4$     & $74.4$      & $78.6$     & $83.7$     & $83.5$ \\
(0, 3) & Stat-w/o    & $93.0$     & $80.9$      & $87.7$     & $93.2$     & $93.2$ \\
& Stat-w/            & $93.0$ \uu & $82.3$ \uu  & $88.1$ \uu & $92.7$ \dd & $92.9$ \dd \\

\hline
& Mean-w/o         & $93.0$     & $83.8$          & $84.9$     & $83.5$     & $88.8$ \\
MM  & Mean-w/      & $90.9$     & $78.1$          & $81.8$     & $74.6$     & $81.3$ \\
(0, 4) & Stat-w/o  & $93.1$     & $83.7$          & $85.3$     & $83.4$     & $88.8$ \\
& Stat-w/ (ours)   & $94.7$ \uu & $\bm{87.5}$ \uu & $87.8$ \uu & $87.9$ \uu & $91.9$ \uu \\

\hline
& Mean-w/o          & $\bm{95.2}$ & $85.9$     & $89.7$       & $91.1$     & $92.5$ \\
MM & Mean-w/        & $94.0$      & $82.1$     & $88.6$       & $87.1$     & $88.9$ \\
(0, 5) & Stat-w/o   & $95.1$      & $85.7$     & $\bm{90.1}$  & $91.1$     & $92.4$ \\
& Stat-w/ (ours)    & $95.0$ \dd  & $86.1$ \uu & $90.1$ \dd   & $91.0$ \dd & $92.2$ \dd \\
\bottomrule
\end{tabular}
\label{table:exp_avmnist_gauss_moda1}
\end{table}

\vspace{6pt}

\noindent \textbf{Results}\quad Table \ref{table:exp_avmnist_gauss_moda1} reports the test accuracies of several models on AV-MNIST. Six unimodal networks are trained on clean data. Then we fuse them with different fusion methods and different robust add-ons. We only invoke our Jacobian regularization for the perturbed audio modality, while keeping the image modality unchanged. First, in the case of mean fusion, confidence-based weighted summation doesn't improve robustness. In the case of statistical fusion, we observe that our proposed Jacobian regularization method not only boosts the accuracy on noisy data but also on clean data. For instance, when our method is invoked on the combination of model-0 and model-1, the test accuracy on clean data increases from  $93.6\%$ to $94.7\%$, and the test accuracy on data with Gaussian noise (e.g., $\omega_0=1.0$) increases from $80.4\%$ to $84.5\%$. Similar phenomena can be observed when our method is invoked on other combinations. Moreover, the number of green arrows is much larger than that of red arrows implying that our method is compatible with different robust techniques and applicable under different noises/attacks.

Comparing the last row in the second sub-section and the third row in the third sub-section, we find that with our proposed method enabled, even if the unimodal backbone model-1 is worse than model-2, the final multimodal accuracies $(0, 1)$ with our method invoked are even larger than $(0, 2)$ without our method invoked. Similar phenomena could usually be observed in other sub-sections. We argue that in this example, statistically fusing two regular unimodal baselines with our Jacobian regularization invoked surpasses robust unimodal baselines and their trivial fusion. Moreover, the highest accuracy in each column has been bolded. It is clear that the multimodal network with our method invoked usually achieves the best performance over all others. The first row of Figure \ref{fig:ablation_diff_gamma} further plots model accuracy versus magnitude of noise/attack. It displays a consistent trend that our method works well regardless of the magnitude of noise/attack. Furthermore, the larger the noise/attack is, the better our method performs. 

\begin{figure}[!thb]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/Picture3.pdf}
    \caption{Accuracies of multimodal networks obtained by statistically fusing a vanilla image network and audio network with $\gamma=0.1$ (the 1-st row), $\gamma=0.5$ (the 2-nd row), and $\gamma=0.9$ (the 3-rd row). Mean and Std of 20 repeated experiments are shown by the solid lines and the shaded regions, respectively. Note that FGSM attack is deterministic, thus there is almost no variance when repeating experiments.}
    \label{fig:ablation_diff_gamma}
\end{figure}

We also plot model accuracy versus magnitude of noise/attack with different gamma values in the second and third row of Figure \ref{fig:ablation_diff_gamma}. Alongside the increasing of $\gamma$, the gap between the orange and blue lines becomes smaller. However, the orange lines consistently appear upon the blue lines, indicating that our method works in a wide range of gamma value and that hyper-parameter tuning is relatively easy in our method. We emphasize that $\gamma=1.0$ is equivalent to trivial fusion.

On the other hand, we consider perturbations on the image modality, while the audio modality is assumed clean. Consequently, we invoke our Jacobian regularization method for the image modality, while keep the audio modality unchanged. We have deliberately enlarged the magnitude of the noise/attack, and results are reported in Table \ref{table:exp_avmnist_gauss_moda2}. As shown in Table \ref{table:exp_avmnist_gauss_moda2}, confidence-weighted summation still doesn't outperform purely mean fusion in all cases. Regards to statistical fusion, the second column demonstrates that this time our Jacobian regularization might lead to accuracy drop on clean data. The phenomenon that robust network is less accurate on clean data might happen as suggested by \cite{robust_at_odds}. However, we notice that such phenomenon doesn't occur in Table \ref{table:exp_avmnist_gauss_moda1}. We believe that such difference might lie intrinsically in modality difference, and we will explore it in our future work.

\begin{table}[!ht]
\small
\centering
\caption{Accuracies of different models (\%) are evaluated on AV-MNIST when image features are perturbed. Mean accuracies are reported after repeatedly running 20 times.}
\vspace{2pt}
\begin{tabular}{clcccccccc}
\toprule
UM / MM & ~~~~Model &  Clean  & $\omega_0 = 2.5$ & $\omega_{2,3} = 10,2$ &  $\omega_4 = 0.07$  &  $\omega_5 = 0.008$\\
\midrule

& 0: Aud-regT       & $83.9$ & $83.9$ & $83.9$ & $83.9$ & $83.9$ \\
& 1: Img-regT       & $73.4$ & $24.4$ & $37.2$ & $15.6$ & $12.3$ \\
UM   & 2: Img-advT  & $73.1$ & $33.4$ & $40.5$ & $43.3$ & $34.1$ \\
Nets & 3: Img-freT  & $65.1$ & $36.2$ & $40.7$ & $46.7$ & $42.6$ \\
& 4: Img-staT       & $74.2$ & $29.5$ & $49.0$ & $19.4$ & $14.1$ \\
& 5: Img-mixT       & $74.1$ & $30.4$ & $37.6$ & $37.3$ & $23.9$ \\
\midrule

&       Mean-w/o    & $93.6$      & $71.9$     & $84.6$      & $83.2$     & $80.0$ \\
MM &  Mean-w/       & $90.5$      & $78.1$     & $83.5$      & $81.6$     & $77.7$ \\
(0, 1) & Stat-w/o   & $93.6$      & $71.7$     & $84.2$      & $83.1$     & $79.9$ \\
&       Stat-w/     & $91.3$ \dd  & $75.2$ \dd & $86.4$ \uu  & $85.4$ \uu & $83.3$ \uu \\

\hline
&       Mean-w/o     & $\bm{93.9}$ & $83.6$     & $85.4$     & $89.9$      & $88.4$ \\
MM &  Mean-w/        & $91.5$      & $82.7$     & $82.0$     & $86.1$      & $83.2$ \\
(0, 2) & Stat-w/o    & $\bm{93.9}$ & $83.5$     & $85.4$     & $\bm{89.9}$ & $88.4$ \\
& Stat-w/   (ours)   & $90.8$ \dd  & $85.0$ \uu & $86.9$ \uu & $88.1$ \dd  & $87.6$ \dd \\

\hline
& Mean-w/o          & $91.4$      & $87.1$          & $88.1$     & $88.8$     & $\bm{88.6}$ \\
MM & Mean-w/        & $88.3$      & $85.6$          & $85.7$     & $85.9$     & $85.5$ \\
(0, 3) & Stat-w/o   & $91.4$      & $87.1$          & $88.2$     & $88.8$     & $\bm{88.6}$ \\
& Stat-w/   (ours)  & $90.9$ \dd  & $\bm{87.0}$ \dd & $88.2$ \uu & $88.6$ \dd & $88.3$ \dd \\

\hline
& Mean-w/o         & $93.7$      & $77.8$     & $89.0$          & $85.1$     & $82.0$ \\
MM  & Mean-w/      & $91.1$      & $83.3$     & $86.8$          & $82.3$     & $78.0$ \\
(0, 4) & Stat-w/o  & $93.7$      & $77.8$     & $89.1$          & $85.0$     & $81.8$ \\
& Stat-w/ (ours)   & $91.3$ \dd  & $79.9$ \dd & $\bm{89.3}$ \uu & $86.4$ \uu & $84.6$ \uu \\

\hline
& Mean-w/o         & $92.6$      & $85.7$      & $86.5$       & $87.2$     & $84.2$ \\
MM & Mean-w/       & $90.1$      & $84.5$      & $84.4$       & $84.3$     & $80.0$ \\
(0, 5) & Stat-w/o  & $92.6$      & $85.7$      & $86.7$       & $87.2$     & $84.1$ \\
& Stat-w/ (ours)   & $92.2$ \dd  & $85.7$ \uu  & $86.9$ \uu   & $87.1$ \dd & $84.6$ \uu \\
\bottomrule
\end{tabular}
\label{table:exp_avmnist_gauss_moda2}
\end{table}


\subsection{Emotion Recognition on RAVDESS}
We consider emotion recognition on RAVDESS \cite{livingstone2018ravdess,xue2021multimodal}. We use a similar network structure for both the image and audio modality: Three convolution layers, two max pooling layers, and three FC layers connect in sequential. Similar baselines and experimental settings are adopted as those in AV-MNIST. Results are reported in Table \ref{table:exp_ravdess_moda1}.

\vspace{6pt}

\noindent\textbf{Results}\quad Still, in the case of mean fusion, confidence-based weighted mean fusion usually doesn't work except in few cases, while our proposed Jacobian regularization exhibits good compatibility with different trained models under various perturbations. The bold results imply that the multimodal network with our Jacobian regularization invoked outperforms all other models except in FGSM attack ($\omega_4=0.03$). Due to page limits, extra results (e.g., perturbation on the image modality) are presented in Supplementary.

% \begin{table}[!ht]
% \small
% \centering
% \caption{Accuracies of different models (\%) are evaluated on RAVDESS when audio features are perturbed. Mean accuracies are reported after repeatedly running 20 times.}
% \vspace{2pt}
% \begin{tabular}{cccccccccc}
% \toprule
% UM / MM & Model &  Clean  & $\omega_0 = 1.0$ & $\omega_1 = 6$ &  $\omega_4 = 0.03$  &  $\omega_5 = 0.001$\\
% \midrule
% & 0: Img-regT       & $82.5$ & $82.5$ & $82.5$ & $82.5$ & $82.5$ \\
% & 1: Aud-regT       & $71.9$ & $54.2$ & $59.3$ & $31.5$ & $29.9$ \\
% UM   & 2: Aud-advT  & $78.6$ & $43.1$ & $71.9$ & $53.3$ & $62.3$\\
% Nets & 3: Aud-freT  & $66.4$ & $19.5$ & $62.4$ & $56.0$ & $60.5$\\
% & 4: Aud-staT       & $71.8$ & $58.3$ & $59.8$ & $25.9$ & $29.6$ \\
% & 5: Aud-mixT       & $74.6$ & $54.5$ & $66.9$ & $15.7$ & $19.2$\\
% \midrule

% & (0,1)-w/o                                                              & $89.9$          & $82.9$          & $86.3$          & $56.9$     & $63.3$ \\
% \rowcolor{gray!20}\cellcolor{white} & (0,1)-w/{\color{gray!20}{o}}       & $89.9$ \uu      & $85.0$ \uu      & $87.7$ \uu      & $59.4$ \uu & $68.1$ \uu\\
% & (0,2)-w/o                                                              & $90.8$          & $77.1$          & $89.6$          & $87.2$     & $90.5$ \\
% \rowcolor{gray!20}\cellcolor{white} & (0,2)-w/{\color{gray!20}{o}}       & $\bm{91.4}$ \uu & $79.9$ \uu      & $\bm{90.2}$ \uu & $88.6$ \uu & $90.6$ \uu \\
% Statistical & (0,3)-w/o                                                  & $90.5$          & $61.5$          & $89.2$          & $\bm{90.0}$& $\bm{90.7}$ \\
% \rowcolor{gray!20}\cellcolor{white} Fusion & (0,3)-w/{\color{gray!20}{o}}& $90.8$ \uu      & $65.6$ \uu      & $90.0$          & $89.5$ \dd & $\bm{90.7}$ \uu\\
% & (0,4)-w/o                                                              & $90.4$          & $88.3$          & $88.5$          & $69.7$     & $78.9$   \\
% \rowcolor{gray!20}\cellcolor{white}      & (0,4)-w/{\color{gray!20}{o}}  & $90.8$ \uu      & $\bm{88.8}$ \uu & $88.7$ \uu      & $75.3$ \uu & $82.3$ \uu \\
% & (0,5)-w/o                                                              & $89.4$          & $87.7$          & $87.9$          & $81.6$     & $82.5$ \\
% \rowcolor{gray!20}\cellcolor{white} & (0,5)-w/{\color{gray!20}{o}}       & $86.6$ \dd      & $86.7$ \dd      & $86.0$ \dd      & $82.9$ \uu & $83.7$ \uu \\
% \midrule

% & (0,1)-w/o                                                              & $89.8$ & $82.8$ & $86.7$  & $57.0$ & $63.6$ \\
% \rowcolor{gray!20}\cellcolor{white} & (0,1)-w/{\color{gray!20}{o}}       & $88.5$ & $80.4$ & $84.1$  & $60.7$ & $57.3$\\
% & (0,2)-w/o                                                              & $90.8$ & $76.9$ & $89.5$  & $87.3$ & $90.6$\\
% \rowcolor{gray!20}\cellcolor{white} & (0,2)-w/{\color{gray!20}{o}}       & $89.3$ & $76.9$ & $87.6$  & $79.7$ & $85.9$\\
% Mean & (0,3)-w/o                                                         & $90.5$ & $60.8$ & $89.6$  & $90.1$ & $90.8$\\
% \rowcolor{gray!20}\cellcolor{white} Fusion & (0,3)-w/{\color{gray!20}{o}}& $86.9$ & $64.0$ & $86.6$  & $82.2$ & $85.7$\\
% & (0,4)-w/o                                                              & $90.7$ & $88.4$ & $88.5$  & $69.3$ & $78.8$\\
% \rowcolor{gray!20}\cellcolor{white} & (0,4)-w/{\color{gray!20}{o}}       & $89.2$ & $85.4$ & $85.5$  & $68.9$ & $69.3$\\
% & (0,5)-w/o                                                              & $89.5$ & $87.8$ & $87.9$  & $81.7$ & $82.7$\\
% \rowcolor{gray!20}\cellcolor{white} & (0,5)-w/{\color{gray!20}{o}}       & $87.9$ & $85.8$ & $86.5$  & $82.0$ & $79.7$\\
% \bottomrule

% \end{tabular}
% \label{table:exp_ravdess_moda1}
% \end{table}

\begin{table}[!ht]
\small
\centering
\caption{Accuracies of different models (\%) are evaluated on RAVDESS when audio features are perturbed. Mean accuracies are reported after repeatedly running 20 times.}
\vspace{2pt}
\begin{tabular}{clcccccccc}
\toprule
UM / MM & ~~~~~Model &  Clean  & $\omega_0 = 1.0$ & $\omega_1 = 6$ &  $\omega_4 = 0.03$  &  $\omega_5 = 0.001$\\
\midrule
& 0: Img-regT       & $82.5$ & $82.5$ & $82.5$ & $82.5$ & $82.5$ \\
& 1: Aud-regT       & $71.9$ & $54.2$ & $59.3$ & $31.5$ & $29.9$ \\
UM   & 2: Aud-advT  & $78.6$ & $43.1$ & $71.9$ & $53.3$ & $62.3$\\
Nets & 3: Aud-freT  & $66.4$ & $19.5$ & $62.4$ & $56.0$ & $60.5$\\
& 4: Aud-staT       & $71.8$ & $58.3$ & $59.8$ & $25.9$ & $29.6$ \\
& 5: Aud-mixT       & $74.6$ & $54.5$ & $66.9$ & $15.7$ & $19.2$\\
\midrule

&       Mean-w/o       & $89.8$     & $82.8$     & $86.7$     & $57.0$     & $63.6$ \\
MM &  Mean-w/          & $88.5$     & $80.4$     & $84.1$     & $60.7$     & $57.3$\\
(0, 1) & Stat-w/o      & $89.9$     & $82.9$     & $86.3$     & $56.9$     & $63.3$ \\
&       Stat-w/ (ours) & $89.9$ \uu & $85.0$ \uu & $87.7$ \uu & $59.4$ \dd & $68.1$ \uu\\

\hline
&       Mean-w/o    & $90.8$          & $76.9$     & $89.5$          & $87.3$     & $90.6$\\
MM &  Mean-w/       & $89.3$          & $76.9$     & $87.6$          & $79.7$     & $85.9$\\
(0, 2) & Stat-w/o   & $90.8$          & $77.1$     & $89.6$          & $87.2$     & $90.5$ \\
& Stat-w/  (ours)   & $\bm{91.4}$ \uu & $79.9$ \uu & $\bm{90.2}$ \uu & $88.6$ \uu & $90.6$ \uu \\

\hline
& Mean-w/o           & $90.5$     & $60.8$     & $89.6$     & $\bm{90.1}$ & $90.8$\\
MM & Mean-w/         & $86.9$     & $64.0$     & $86.6$     & $82.2$      & $85.7$\\
(0, 3) & Stat-w/o    & $90.5$     & $61.5$     & $89.2$     & $90.0$      & $90.7$ \\
& Stat-w/ (ours)     & $90.8$ \uu & $65.6$ \uu & $90.0$ \uu & $89.5$ \dd  & $\bm{90.7}$ \dd\\

\hline
& Mean-w/o         & $90.7$     & $88.4$          & $88.5$      & $69.3$     & $78.8$\\
MM  & Mean-w/      & $89.2$     & $85.4$          & $85.5$      & $68.9$     & $69.3$\\
(0, 4) & Stat-w/o  & $90.4$     & $88.3$          & $88.5$      & $69.7$     & $78.9$   \\
& Stat-w/ (ours)   & $90.8$ \uu & $\bm{88.8}$ \uu & $88.7$ \uu  & $75.3$ \uu & $82.3$ \uu \\

\hline
& Mean-w/o          & $89.5$      & $87.8$     & $87.9$     & $81.7$     & $82.7$\\
MM & Mean-w/        & $87.9$      & $85.8$     & $86.5$     & $82.0$     & $79.7$\\
(0, 5) & Stat-w/o    & $89.4$      & $87.7$     & $87.9$     & $81.6$     & $82.5$ \\
& Stat-w/ (ours)    & $86.6$ \dd  & $86.7$ \dd & $86.0$ \dd & $82.9$ \uu & $83.7$ \uu \\
\bottomrule
\end{tabular}
\label{table:exp_ravdess_moda1}
\end{table}


\subsection{VGGSound}


% \begin{table}[!ht]
% \small
% \centering
% \caption{Accuracies of different models (\%) are evaluated on VGGSound when video features are perturbed. Mean accuracies are reported after repeatedly running 5 times. Each gray-shaded row in the statistical fusion subsection shares the same $\gamma$, and its value is selected from $\{0.1,0.5,0.9\}$.}
% \vspace{2pt}
% \begin{tabular}{cccccccccc}
% \toprule
% UM / MM & Model &  Clean  & $\omega_0 = 1.5$ & $\omega_1 = 6$ &  $\omega_4 = 0.03$  &  $\omega_5 = 0.001$\\
% \midrule
% & 0: Aud-regT       & $54.4$ & $15.0$ & $49.8$ & $23.0$ & $19.9$ \\
% & 1: Img-regT       & $27.4$ & $5.8$ & $27.4$ & $9.5$ & $9.0$ \\
% UM   & 2: Img-advT  & $27.5$ & $5.3$ & $27.4$ & $10.7$ & $10.3$\\
% Nets & 3: Img-freT  & $25.2$ & $4.0$ & $24.2$ & $20.4$ & $22.9$\\
% & 4: Img-staT       & $27.0$ & $6.9$ & $26.9$ & $10.5$ & $9.6$ \\
% & 5: Img-mixT       & $27.2$ & $8.4$ & $27.1$ & $7.3$ & $7.2$\\
% \midrule

% & (0,1)-w/o                                                              & $58.5$          & $46.0$          & $58.4$          & $35.3$     & $26.0$ \\
% \rowcolor{gray!20}\cellcolor{white} & (0,1)-w/{\color{gray!20}{o}}       & $60.1$ \uu      & $51.2$ \uu      & $60.0$ \uu      & $39.7$ \uu & $28.5$ \uu\\
% & (0,2)-w/o                                                              & $59.4$          & $45.4$          & $59.4$          & $37.2$     & $27.2$ \\
% \rowcolor{gray!20}\cellcolor{white} & (0,2)-w/{\color{gray!20}{o}}       & $\bm{61.1}$ \uu & $50.1$ \uu      & $\bm{61.1}$ \uu & $41.2$ \uu & $29.7$ \uu \\
% Statistical & (0,3)-w/o                                                  & $58.8$          & $52.6$          & $58.8$          & $55.6$& $57.7$ \\
% \rowcolor{gray!20}\cellcolor{white} Fusion & (0,3)-w/{\color{gray!20}{o}}& $56.7$ \dd      & $53.2$ \uu      & $56.7$ \dd & $\bm{58.5}$ \uu & $\bm{57.9}$ \uu\\
% & (0,4)-w/o                                                              & $58.2$          & $47.5$          & $58.1$          & $37.4$     & $31.0$   \\
% \rowcolor{gray!20}\cellcolor{white}      & (0,4)-w/{\color{gray!20}{o}}  & $59.8$ \uu      & $51.9$ \uu & $59.7$ \uu      & $41.0$ \uu & $34.0$ \uu \\
% & (0,5)-w/o                                                              & $59.1$          & $\bm{56.4}$          & $59.0$          & $54.5$     & $54.3$ \\
% \rowcolor{gray!20}\cellcolor{white} & (0,5)-w/{\color{gray!20}{o}}       & $57.1$ \dd      & $55.9$ \dd      & $57.0$ \dd      & $55.2$ \uu & $55.4$ \uu \\
% \midrule

% & (0,1)-w/o                                                              & $57.7$ & $45.8$ & $57.7$  & $35.0$ & $25.7$ \\
% \rowcolor{gray!20}\cellcolor{white} & (0,1)-w/{\color{gray!20}{o}}       & $53.9$ & $48.6$ & $53.9$  & $37.9$ & $20.5$\\
% & (0,2)-w/o                                                              & $58.8$ & $45.0$ & $58.8$  & $37.2$ & $26.9$\\
% \rowcolor{gray!20}\cellcolor{white} & (0,2)-w/{\color{gray!20}{o}}       & $54.1$ & $49.0$ & $54.1$  & $38.3$ & $21.3$\\
% Mean & (0,3)-w/o                                                         & $57.9$ & $51.5$ & $57.9$  & $57.8$ & $57.7$\\
% \rowcolor{gray!20}\cellcolor{white} Fusion & (0,3)-w/{\color{gray!20}{o}}& $55.2$ & $53.6$ & $55.2$  & $55.0$ & $55.2$\\
% & (0,4)-w/o                                                              & $57.5$ & $47.2$ & $57.3$  & $36.9$ & $30.9$\\
% \rowcolor{gray!20}\cellcolor{white} & (0,4)-w/{\color{gray!20}{o}}       & $53.5$ & $49.2$ & $53.4$  & $37.2$ & $23.4$\\
% & (0,5)-w/o                                                              & $57.8$ & $55.3$ & $57.8$  & $53.9$ & $53.5$\\
% \rowcolor{gray!20}\cellcolor{white} & (0,5)-w/{\color{gray!20}{o}}       & $55.6$ & $54.7$ & $55.6$  & $54.3$ & $49.5$\\
% \bottomrule

% \end{tabular}
% \label{table:exp_vggsound_moda1}
% \end{table}


\begin{table}[!ht]
\small
\centering
\caption{Accuracies of different models (\%) are evaluated on VGGSound when video features are perturbed. Mean accuracies are reported after repeatedly running 5 times.}
\vspace{2pt}
\begin{tabular}{clcccccccc}
\toprule
UM / MM & ~~~~~Model &  Clean  & $\omega_0 = 1.5$ & $\omega_1 = 6$ &  $\omega_4 = 0.03$  &  $\omega_5 = 0.001$\\
\midrule
& 0: Aud-regT       & $54.4$ & $15.0$ & $49.8$ & $23.0$ & $19.9$ \\
& 1: Img-regT       & $27.4$ & $5.8$ & $27.4$ & $9.5$ & $9.0$ \\
UM   & 2: Img-advT  & $27.5$ & $5.3$ & $27.4$ & $10.7$ & $10.3$\\
Nets & 3: Img-freT  & $25.2$ & $4.0$ & $24.2$ & $20.4$ & $22.9$\\
& 4: Img-staT       & $27.0$ & $6.9$ & $26.9$ & $10.5$ & $9.6$ \\
& 5: Img-mixT       & $27.2$ & $8.4$ & $27.1$ & $7.3$ & $7.2$\\
\midrule
&       Mean-w/o        & $57.7$ & $45.8$ & $57.7$  & $35.0$ & $25.7$ \\
MM &  Mean-w/           & $53.9$ & $48.6$ & $53.9$  & $37.9$ & $20.5$\\
(0, 1) & Stat-w/o       & $58.5$ & $46.0$ & $58.4$  & $35.3$ & $26.0$ \\
&       Stat-w/  (ours) & $60.1$ \uu      & $51.2$ \uu      & $60.0$ \uu     & $39.7$ \uu & $28.5$ \uu\\

\hline
&       Mean-w/o      & $58.8$ & $45.0$ & $58.8$  & $37.2$ & $26.9$\\
MM &  Mean-w/         & $54.1$ & $49.0$ & $54.1$  & $38.3$ & $21.3$\\
(0, 2) & Stat-w/o     & $59.4$ & $45.4$ & $59.4$  & $37.3$ & $27.2$ \\
& Stat-w/ (ours)      & $\bm{61.1}$ \uu & $50.1$ \uu      & $\bm{61.1}$ \uu & $41.2$ \uu & $29.7$ \uu \\

\hline
& Mean-w/o          & $57.9$ & $51.5$ & $57.9$  & $57.8$ & $57.7$\\
MM & Mean-w/        & $55.2$ & $53.6$ & $55.2$  & $55.0$ & $55.2$\\
(0, 3) & Stat-w/o   & $58.8$ & $52.6$ & $58.8$  & $55.6$ & $57.7$ \\
& Stat-w/  (ours)   & $56.7$ \dd      & $53.2$ \dd      & $56.7$ \dd & $\bm{58.5}$ \uu & $\bm{57.9}$ \uu\\

\hline
& Mean-w/o          & $57.5$ & $47.2$ & $57.3$  & $36.9$ & $30.9$\\
MM  & Mean-w/       & $53.5$ & $49.2$ & $53.4$  & $37.2$ & $23.4$\\
(0, 4) & Stat-w/o   & $58.2$ & $47.5$ & $58.1$  & $37.4$ & $31.0$   \\
& Stat-w/ (ours)    & $59.8$ \uu      & $51.9$ \uu & $59.7$ \uu      & $41.0$ \uu & $34.0$ \uu \\

\hline
& Mean-w/o          & $57.8$ & $55.3$      & $57.8$  & $53.9$ & $53.5$\\
MM & Mean-w/        & $55.6$ & $54.7$      & $55.6$  & $54.3$ & $49.5$\\
(0, 5) & Stat-w/o   & $59.1$ & $\bm{56.4}$ & $59.0$  & $54.5$ & $54.3$ \\
& Stat-w/ (ours)    & $57.1$ \dd      & $55.9$ \dd      & $57.0$ \dd      & $55.2$ \uu & $55.4$ \uu \\
\bottomrule
\end{tabular}
\label{table:exp_vggsound_moda1}
\end{table}

We consider classification task on a real-world data set VGGSound~\cite{chen2020vggsound}, where two modalities audio and video are available. To construct an affordable problem, our classification task only focuses on a subset of all classes. Namely, we randomly choose 100 classes and our classification problem is constrained on them. Consequently, there are 53622 audio-video pairs for training and 4706 audio-video pairs for testing. For the audio modality, we apply a short-time Fourier transform on each raw waveform, generating a 313 $\times$ 513 spectrogram. We take a 2D ResNet-18~\cite{resnet} to process these spectrograms. For the video modality, we evenly sample 32 frames from each 10-second video resulting input feature size of 32 $\times$ 256 $\times$ 256. We take a ResNet-18 network to process the video input where 3D convolutions have been adopted to replace 2D convolutions.

\vspace{6pt}

\noindent\textbf{Results} We present the results of mean fusion and statistical fusion with or without robust add-on in Table \ref{table:exp_vggsound_moda1}. Unlike the previous experiments, here we make audio modality clean and assume corruptions/attacks on the video modality. The results demonstrate that our method outperforms counterpart statistical fusion without Jacobian regularization in most cases. Furthermore, the bold results imply that our Jacobian regularization could enhance model robustness under various corruptions or attacks. {In Supplementary, we capture another important setting: the video modality (or audio modality) is corrupted, but we don't know which one.} Thus, both modalities are trained with robust add-ons. Please refer to Supplementary for more details.
